Stream-R1: Reliability-Perplexity Aware Reward Distillation for Streaming Video Generation

Distillation-based acceleration has become foundational for making autoregressive streaming video diffusion models practical, with distribution matching distillation (DMD) as the de facto choice. Existing methods, however, train the student to match the teacher's output indiscriminately, treating every rollout, frame, and pixel as equally reliable supervision. We argue that this caps distilled quality, since it overlooks two complementary axes of variance in DMD supervision: Inter-Reliability across student rollouts whose supervision varies in reliability, and Intra-Perplexity across spatial regions and temporal frames that contribute unequally to where quality can still be improved. The objective thus conflates two questions under a uniform weight: whether to learn from each rollout, and where to concentrate optimization within it. To address this, we propose Stream-R1, a Reliability-Perplexity Aware Reward Distillation framework that adaptively reweights the distillation objective at both rollout and spatiotemporal-element levels through a single shared reward-guided mechanism. At the Inter-Reliability level, Stream-R1 rescales each rollout's loss by an exponential of a pretrained video reward score, so that rollouts with reliable supervision dominate optimization. At the Intra-Perplexity level, it back-propagates the same reward model to extract per-pixel gradient saliency, which is factored into spatial and temporal weights that concentrate optimization pressure on regions and frames where refinement yields the largest expected gain. An adaptive balancing mechanism prevents any single quality axis from dominating across visual quality, motion quality, and text alignment. Stream-R1 attains consistent improvements on all three dimensions over distillation baselines on standard streaming video generation benchmarks, without architectural modification or additional inference cost.

==> sec/6_exps_ab.tex <==
\newpage
\section{Ablation Study}

\subsection{Effect of Style Reward Learning (SRL). }
\noindent \textbf{For style-driven task:} As shown in~\Cref{fig7_2:comparison_ab_srl}, the last three columns reveal a clear boost in style similarity for both style-driven and style-subject-driven tasks; the stroke textures and painting style closely match the reference images, confirming the effectiveness of our style reward learning.

\noindent \textbf{For subject-driven task:} In the first three and final columns of~\Cref{fig7_2:comparison_ab_srl}, we observe a notable improvement in subject and identity consistency, with more uniform details and higher facial similarity.

As shown in~\Cref{tab:main_ab}, removing SRL leads to a sharp drop in the CSD score and simultaneous declines in CLIP-I and CLIP-T. Notably, we rely solely on style reward and introduce no identity-specific data; nevertheless, the unified model benefits in content consistency. By sharpening the model’s ability to extract and retain desired features, SRL yields an overall improvement across all tasks, strongly validating our motivation. Beyond gains in subject and identity fidelity, we observe a noticeable enhancement in aesthetic quality (e.g., texture as in VMix~\cite{wu2024vmix}) and a marked reduction in the plastic artifact, which is an issue that has long challenged text-to-image generation~\cite{wu2024vmix}. Through SRL training, the model exhibits emerging properties even in tasks not explicitly targeted during training.

\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{figs/comparison_ab_srl.pdf}
    \caption{Ablation study of SRL. The \textcolor{mytextblue}{blue} boxes denote content reference and the \textcolor{mypurple}{purple} boxes denote style reference. Prompts are "A toy with a mountain in the background.", "The man on the beach.", "The woman is skateboarding on the street.", "A beautiful woman.", "A beautiful woman.", "The woman gave an impassioned speech on the podium." from left to right.}
    \label{fig7_2:comparison_ab_srl}
\end{figure*}
\input{tables/ablations.tex}

\subsection{Effect of Style Alignment Training (SAT).}
Removing SAT and instead jointly fine-tuning both SigLIP and DiT from scratch degrades CLIP-T on subject-driven tasks and lowers CSD on style-subject-driven tasks (~\Cref{tab:main_ab}). Qualitatively, ~\Cref{fig7:comparison_ab} shows that the oil-painting style of the “cheetah” example becomes noticeably weaker.

\begin{figure}[t]
\centering
\includegraphics[width=0.85\textwidth]{figs/comparison_ab.pdf}
    \caption{Ablation study of USO. Zoom in for details.}
    \label{fig7:comparison_ab}
\end{figure}

\subsection{Effect of Disentangled Encoder (DE).}
Replacing the disentangled encoders with a single VAE for both style and content images harms nearly every metric (~\Cref{tab:main_ab}). Visually, the “cheetah” reverts to a more photorealistic appearance, while the man’s identity suffers a marked loss (~\Cref{fig7:comparison_ab}).

\subsection{Effect of Hierarchical Projector.} ~\Cref{tab:stage1_ab} shows that the hierarchical projector yields the highest CSD and a leading CLIP-T score, substantially benefiting style-alignment training.

==> sec/8_sup.tex <==
% \clearpage
% \setcounter{page}{12}



% 添加附录标题
\onecolumn
\section*{\centering\LARGE\bfseries NativeTok: Native Visual Tokenization for Improved Image Generation}
\section*{\centering Appendix}
% 自定义 section 和 subsection 的编号格式
\renewcommand{\thesection}{\Alph{section}}
\renewcommand{\thesubsection}{\Alph{section}.\arabic{subsection}}

\subsection{Training and Testing Protocols} \label{sec:intro}
\renewcommand{\arraystretch}{0.7}
\begin{table}[H]
\centering
\begin{tabular}{l|l}
\textbf{Configuration} & \textbf{Value} \\

\hline
\multicolumn{2}{c}{\textit{NativeTok$_{32}$}} \\
Meta Image Transformer layers & 18 \\
Meta Image Transformer dim & 1024 \\
MoCET layers & 32 \\
MoCET dim & 256 \\
decoder layers & 24 \\
decoder dim & 1024 \\
total parameters & 616M \\
training strategy & full param training \\
Trainable params rate & 100\% \\
speed & 63.44/s/gpu Batch \\
\hline
\multicolumn{2}{c}{\textit{NativeTok$_{64}$}} \\
Meta Image Transformer layers & 18 \\
Meta Image Transformer dim & 1024 \\
MoCET layers & 64 \\
MoCET dim & 256 \\
decoder layers & 24 \\
decoder dim & 1024 \\
total parameters & 666M \\
training strategy & HNT strategy \\
Trainable params rate & 56\% \\
speed & 54.14/s/gpu Batch \\
speed of full parameter fine-tune & 40.48/s/gpu Batch \\
\hline
\multicolumn{2}{c}{\textit{NativeTok$_{128}$}} \\

Meta Image Transformer layers & 18 \\
Meta Image Transformer dim & 1024 \\
MoCET layers & 128 \\
MoCET dim & 256 \\
decoder layers & 24 \\
decoder dim & 1024 \\
total parameters & 766M \\
training strategy & HNT strategy \\
Trainable params rate & 55\% \\
speed & 39.44/s/gpu Batch \\
speed of full parameter fine-tune & 30.75/s/gpu Batch \\
\hline
\multicolumn{2}{c}{\textit{Training Configuration}} \\

dateset & ImageNet1K \\
image resolution & 256\(\times\)256 \\
random crop& True\\
random flip& True\\
device & NVIDIA A800 $\times$ 4  \\
per gpu batch size & 64 \\
global batch size & 256 \\
optimizer & AdamW  \\
base learning rate & \(1\text{e}^{-4}\) \\
learning rate schedule & cosine \\
end learning rate & \(1\text{e}^{-5}\) \\
warmup steps & 5K \\
weight decay & \(1\text{e}^{-4}\) \\
optimizer momentum & \(\beta_1, \beta_2 = 0.9,\ 0.99\) \\
training steps & 500K \\
\hline
\end{tabular}
\caption{Configuration of NativeTok. } 
\label{tab:config}
\end{table}
\renewcommand{\arraystretch}{1} % 恢复默认值
For image generation using \textbf{NativeTok}, we provide the configuration and training strategies across three model scales: \textit{NativeTok$_{32}$}, \textit{NativeTok$_{64}$}, and \textit{NativeTok$_{128}$}. All models are trained on ImageNet-1K at resolution \(256 \times 256\) with center cropping and horizontal flipping as the only augmentations.

\textbf{For \textit{NativeTok$_{32}$}}, we use a Meta Image Transformer with 18 layers and 1024 hidden dimensions, followed by a Mixture of Causal Expert Transformer composed of 32 layers with 256 hidden dimensions. The decoder has 24 layers and 1024 hidden dimensions. This model contains a total of 616M parameters and is trained with full parameter updates. The training throughput is 63.44 samples per second per GPU.

\textbf{For \textit{NativeTok$_{64}$}}, we increase the Mixture of Causal Expert Transformer to 64 layers while keeping other components unchanged. The model size grows to 666M parameters. We employ the Hierarchical Native Training (HNT) strategy over 450K training steps, resulting in only 56\% of parameters being updated during initial training. The training speed is 54.14 samples/s/GPU, and 40.48 samples/s/GPU for full-parameter fine-tuning.

\textbf{For \textit{NativeTok$_{128}$}}, we maintain the same architecture as \textit{NativeTok$_{64}$} but scale the training to a larger Mixture of Experts model with the same 64 expert layers. The parameter count rises to 766M. HNT strategy is used again with 55\% trainable parameters. Training throughput is 39.44 samples/s/GPU, dropping to 30.75 samples/s/GPU for full fine-tuning.

\textbf{Training configuration.} All models are trained using 4 NVIDIA A800 GPUs with a per-GPU batch size of 64 (global batch size 256). We use the AdamW optimizer with \(\beta_1 = 0.9\), \(\beta_2 = 0.99\), a base learning rate of \(1 \times 10^{-4}\), cosine decay schedule down to \(1 \times 10^{-5}\), and weight decay of \(1 \times 10^{-4}\). The warm-up phase lasts 5K steps, and the full training takes 500K steps.

\textbf{Hierarchical Native Training strategy.} For larger model variants (\textit{NativeTok$_{64}$} and \textit{NativeTok$_{128}$}), we use the Hierarchical Native Training (HNT) strategy, which gradually expands trainable parameter subsets to mitigate optimization difficulty in large-scale mixtures of experts.

We provide the complete configuration in table~\ref{tab:config}.




\subsection{Detailed Results of Preliminary Experiments} \label{sec:related}
\begin{table}[H]
\centering
% 第一个表格
\renewcommand{\arraystretch}{}
\setlength{\tabcolsep}{1pt}
{
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcc@{}}
\toprule
\textbf{Model} & \textbf{Params$\downarrow$} & \textbf{rFID$\downarrow$} \\
\midrule
\multicolumn{3}{c}{stage1} \\
NativeTok$_{32}$ & 616M & 5.10 \\
NativeTok$_{64}$& 666M & 3.54 \\
NativeTok$_{128}$ & 766M & 2.86 \\
 \hline
 \multicolumn{3}{c}{add decoder finetune} \\

NativeTok$_{32}$ & 616M & 2.57 \\
NativeTok$_{64}$& 666M & 1.89 \\
NativeTok$_{128}$ & 766M & 1.19 \\
\bottomrule

\end{tabular*}
\caption{Detailed Performance of NativeTok.}
\label{generator}

}
\hfill

\hfill


\end{table}
\textbf{Detailed Performance of NativeTok.} We report the performance of different NativeTok variants across both training stages, as summarized in Table~\ref{generator}.

To quantitatively assess reconstruction quality, we measure rFID scores (lower is better) under two settings: \textit{Stage 1 only} and \textit{Stage 1 + decoder fine-tuning}. As shown in Table~\ref{generator}, increasing model capacity from NativeTok$_{32}$ to NativeTok$_{128}$ consistently enhances reconstruction quality. Under Stage 1 alone, the rFID decreases from 5.10 to 2.86 with increasing model scale. With additional decoder fine-tuning, the rFID further improves to 2.57, 1.89, and 1.19 for NativeTok$_{32}$, NativeTok$_{64}$, and NativeTok$_{128}$, respectively.

In addition, the parameter count reflects the impact of increasing the number of experts in the MoCET module. Although larger token counts result in more MoCET parameters, the increase is sublinear: every additional 32 tokens introduce only about an 8\% increase in parameters relative to the base model.




\subsection{Qualitative Visualization} \label{sec:method}

We provide more detailed quantitative metrics corresponding to the visualization section in the main paper in Table~\ref{overlap_comparison}. Specifically, we modify short token subsequences of varying lengths from 1 to 4 and compute the average top-100 overlap rate across 1,000 ImageNet classes. We compare the results of NativeTok and TiTok under the same setting. The results show that NativeTok consistently exhibits a lower overlap rate, indicating that the generator is more sensitive to token-level variations. This reflects a stronger alignment between the token representations and the generation behavior, resulting in more precise outputs.




We provide several reconstruction visualizations in Figure~\ref{fig:recon}. From left to right: original image, NativeTok$_{128}$ reconstruction, NativeTok$_{64}$ reconstruction, and NativeTok$_{32}$ reconstruction.

\begin{table}[H]
\centering

\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{12pt}
\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} 
                >{\centering\arraybackslash}m{1.8cm} 
                >{\centering\arraybackslash}m{1.8cm}}
\toprule
\footnotesize\textbf{Number of Inconsistent Tokens} & 
\footnotesize\textbf{NativeTok Overlap Ratio} & 
\footnotesize\textbf{TiTok Overlap Ratio} \\
\midrule
1 & 56.26\% & 78.66\% \\
2 & 50.89\% & 75.78\% \\
3 & 48.34\% & 73.43\% \\
4 & 48.44\% & 68.37\% \\
\bottomrule
\end{tabular}
\caption{Comparison of Token Overlap Ratios between NativeTok and TiTok.}
\label{overlap_comparison}
\end{table}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{fig/visiualiation2.pdf}
    \caption{Reconstructions during the token generation process where the token count increases from 0 to 32.}
    \label{fig:process}
\end{figure*}
In Figure~\ref{fig:process}, we visualize the morphological changes of NativeTok$_{32}$ and Titok$_{32}$ reconstructions during the token generation process where the token count increases from 0 to 32. Our observations reveal that: Under Titok$_{32}$'s bidirectional attention mechanism, earlier tokens inherently contain information from subsequent tokens. In contrast, NativeTok$_{32}$ with unidirectional attention progressively incorporates novel visual information not present in previous tokens.

We provide several qualitative examples of generated images in Figure~\ref{fig:Generation}.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/recon.pdf}
    \caption{We provide a demonstration of reconstruction results. From left to right: the original image, reconstruction image by NativeTok$_{128}$, reconstruction image by NativeTok$_{64}$, and reconstruction image by NativeTok$_{32}$.}
    \label{fig:recon}
\end{figure*}





\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{fig/generater.pdf}
    \caption{Generation examples}
    \label{fig:Generation}
\end{figure*}

\subsection{Limitations}
While our proposed method demonstrates promising performance in both reconstruction and generation tasks, several limitations remain to be addressed in future work.

\textbf{Two-stage Training Pipeline.}
Similar to previous methods such as TiTok, our framework still adopts a two-stage training scheme, where the image tokenizer is trained independently from the autoregressive generative model. Although we partially alleviate the gap between these stages through hierarchical causal training and decoder fine-tuning, a fully unified end-to-end training pipeline remains unexplored. Bridging this gap could further improve token quality and model coherence, especially in downstream autoregressive tasks.

\textbf{Limited Training Scale.}
Due to computational constraints and limited resources, we were only able to train the autoregressive generator using the smallest variant, \textit{NativeTok}${32}$. While this variant already shows clear advantages over its TiTok counterpart, it does not fully exploit the benefits of higher-capacity tokenizers like \textit{NativeTok}${128}$. As a result, our generation results may not reflect the upper bound of our proposed framework's potential. Future work will include large-scale training of the autoregressive model on more capable tokenizer variants, which is expected to yield further improvements.



==> tables/ablations.tex <==
\begin{figure}[thb]
\CenterFloatBoxes
\begin{floatrow}

% Left Table
\ttabbox
{
\resizebox{\linewidth}{!}{
    \begin{tabular}{lcc|cc}
    \toprule
    \textbf{Model} & \multicolumn{2}{c|}{\textbf{Subject-driven}} & \multicolumn{2}{c}{\textbf{Style-subject-driven}} \\
    
    % \cmidrule(lr){3-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-15}
    &CLIP-I$\uparrow$ & CLIP-T$\uparrow$ & CSD$\uparrow$ & CLIP-T$\uparrow$ \\
    \midrule
    \textbf{USO (Ours)} & \textbf{0.623} & \textbf{0.288} & \textbf{0.495} & \textbf{0.283}  \\
    \midrule
    w/o SRL & 0.620 & \underline{0.284}  & \underline{0.413} & \underline{0.280} \\
    w/o SAT & \underline{0.621} & 0.275 & 0.409 & \underline{0.280}\\
    w/o DE & 0.594 & 0.269 & 0.382 & 0.277 \\
    \bottomrule
    \end{tabular}
}}
{\caption{Ablation study of different components proposed in USO. }
 \label{tab:main_ab}
}

% Right Table
\ttabbox
{
\resizebox{0.965\linewidth}{!}{
    \begin{tabular}{lcc}
    \toprule
    \textbf{Model} & CSD$\uparrow$ & CLIP-T$\uparrow$ \\
    \midrule

    resampler (depth=1) & \underline{0.336} & 0.279 \\
    resampler, unfreeze siglip & 0.155 & \textbf{0.288} \\
    mlp (depth=1) & 0.277 & \underline{0.284} \\
    mlp, unfreeze siglip & 0.179 & \textbf{0.288} \\
    hierarchical projector & \textbf{0.402} & \underline{0.284} \\

    \bottomrule
    \end{tabular}
}}
{\caption{Ablation study of different projector in USO.}
 \label{tab:stage1_ab}
}

\end{floatrow}
\end{figure}


==> tables/dreambench.tex <==
\begin{table*}[t]
\centering
\small
% \resizebox*{0.425\textwidth}{!}{
% \resizebox*{0.5\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Method} & \textbf{DINO} $\uparrow$ & \textbf{CLIP-I} $\uparrow$ & \textbf{CLIP-T} $\uparrow$ \\ \toprule
Oracle(reference images) & 0.774 & 0.885 & - \\\hline
Textual Inversion \cite{gal2022image} & 0.569 & 0.780 & 0.255\\
DreamBooth \cite{ruiz2023dreambooth} &0.668  & 0.803 & 0.305 \\
BLIP-Diffusion \cite{li2023blip} & 0.670 & 0.805 & 0.302\\\hline
ELITE \cite{wei2023elite}& 0.647  & 0.772 & 0.296\\
Re-Imagen \cite{chen2022re}& 0.600  & 0.740 & 0.270\\
BootPIG\cite{purushwalkam2024bootpig} & 0.674  & 0.797 & 0.311\\
SSR-Encoder\cite{zhang2024ssr} & 0.612  & 0.821 & 0.308\\
RealCustom++ \cite{huang2024realcustom, mao2024realcustom++}& 0.702  & 0.794 & \textbf{0.318}\\
OmniGen \cite{xiao2024omnigen}& 0.693  & 0.801 & 0.315\\
OminiControl \cite{tan2024ominicontrol}& 0.684  & 0.799 & 0.312\\
FLUX.1 IP-Adapter & 0.582  & 0.820 & 0.288\\
UNO~\cite{wu2025less} & \underline{0.760}  & \underline{0.835} & 0.304\\
\rowcolor{myblue} \textbf{USO (Ours)} & \textbf{0.777} & \textbf{0.838} & \underline{0.317} \\
\bottomrule
\end{tabular}
%}
\caption{Quantitative results for single-subject driven generation on Dreambench~\cite{ruiz2023dreambooth}.}
\label{tab1:sup_dreambench}
\end{table*}

==> tables/main_res.tex <==
\begin{table*}[h]
    \centering
    % \resizebox{0.99\linewidth}{31.5mm}{
    \resizebox{0.86\linewidth}{!}{
        \begin{tabular}{lccc|cc}
        \toprule
        \textbf{Model} & \multicolumn{3}{c|}{\textbf{Subject-driven generation}} & \multicolumn{2}{c}{\textbf{Style-driven generation}}\\
        
        % \cmidrule(lr){3-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-15}
        &CLIP-I$\uparrow$ & DINO$\uparrow$ & CLIP-T$\uparrow$ & CSD$\uparrow$ & CLIP-T$\uparrow$  \\
        \midrule
        % \multicolumn{14}{l}{\textit{Image Understanding}} \\
        RealCustom++~\cite{huang2024realcustom} & 0.314 & 0.615 & \textbf{0.303} & - & - \\
        RealGeneral~\cite{lin2025realgeneral} & 0.485 & 0.732 & 0.275  & - & -\\
        UNO~\cite{wu2025less} & \underline{0.605} & \underline{0.789} & 0.264  & - & -\\
        BAGEL~\cite{deng2025emerging}  & 0.516 & 0.741 & 0.298 & - & -\\ 
        OmniGen2~\cite{wu2025omnigen2} & 0.475 & 0.723 & \underline{0.302}  & - & -\\
        FLUX.1 Kontext dev~\cite{labs2025flux} & 0.579 & 0.775 & 0.287  & - & -\\
        Qwen-Image Edit~\cite{wu2025qwen} & 0.544 & 0.756 & \underline{0.302}  & - & -\\
        \midrule
        % \multicolumn{14}{l}{\textit{Text-to-Image Generation}} \\
        DEADiff~\cite{qi2024deadiff} & - & - & - & 0.462 & 0.274 \\
        InstantStyle-XL~\cite{wang2024instantstyle} & - & - & - & \underline{0.540} & 0.276 \\
        CSGO~\cite{xing2024csgo} & - & - & - & 0.452 & 0.272 \\
        StyleStudio~\cite{lei2025stylestudio}  & - & - & - & 0.348 & \textbf{0.282} \\
        \midrule
        DreamO~\cite{mou2025dreamo} & 0.588 & 0.787 & 0.280  & 0.454 & \underline{0.278} \\
        \midrule
        \rowcolor{myblue} \textbf{USO (Ours)}  & \textbf{0.623} & \textbf{0.793} & 0.288 & \textbf{0.557} & \textbf{0.282} \\

        \bottomrule
        \end{tabular}
}
     \caption{Quantitative results for subject-driven and style-driven generation on USO-Bench.}
    \label{tab:main_comparison}
\end{table*}

==> tables/main_res2.tex <==
\begin{table}[h]
    \centering
    % \resizebox{0.99\linewidth}{31.5mm}{
    \resizebox{0.38\linewidth}{!}{
        \begin{tabular}{lcc}
        \toprule
        \textbf{Model} & CSD$\uparrow$ & CLIP-T$\uparrow$ \\
        \midrule
        StyleID~\cite{chung2024style} & \underline{0.407} & \underline{0.230} \\
        OmniStyle~\cite{wang2025omnistyle} & 0.365 & 0.229 \\
        \midrule
        \rowcolor{myblue} \textbf{USO (Ours)}  & \textbf{0.495} & \textbf{0.283} \\
        \bottomrule
        \end{tabular}
}
     \caption{Quantitative results for style-subject-driven driven generation on USO-Bench.}\label{tab:ip_style_comparison}
\end{table}

==> tables/srl.tex <==
% \begin{algorithm}[tb]
% \caption{Style Reward Learning (SRL) with Flow Matching}
% \begin{algorithmic}[1] %[1] enables line numbers
% \Require Customization models $v$ with pretrained parameters $\theta$; pretrain loss function $\mathcal{L}_{\text{Pre}}$; reward function $\mathcal{L}_{\text{SRL}}$; reward model $\mathcal{M}_{\text{RM}}$; balancing coefficient $\lambda$; the number of noise scheduler time steps $T$; time step range for SRL finetuning $[t_s,t_e]$; Dataset $\mathcal{D}=\{(y,I_0,I^c_{ref},I^s_{ref})_i\mid i=1,2,\dots\}$, $y$ is prompt, $I_0$ is target image and $I^c_{ref},I^s_{ref}$ are reference content and style images (\Cref{uno_dataset})

% \FOR{$(y_i,I_0,I^c_{ref},I^s_{ref})\in\mathcal{D}$}
%     \STATE $\mathcal{L}_{\text{Pre}} \gets v_{\theta}(y_i,I_0,I^c_{ref},I^s_{ref})$ // Calculate pretrained loss with condition
%     \STATE $t \gets \mathcal{U}(t_s,t_e)$ // Pick a random time step in $[t_s,t_e]$
%     \STATE $x_T \sim \mathcal{N}(0, I)$
%     \FOR{$\tau=T,\dots,t+1$}
%         \STATE $\hat{v}_{\tau+1}\gets \text{no\_grad}(v_{\theta}(y_i,x_{\tau+1},I^c_{ref},I^s_{ref}))$
%         \STATE $\hat{I}_{t}\gets \hat{v}_{\tau+1}$
%     \ENDFOR
%     \STATE $\hat{v}_{t}\gets v_{\theta}(y_i,x_{t+1},I^c_{ref},I^s_{ref})$
%     \STATE $\hat{I}_{0}\gets v_{t}$ // Predict original image
%     \STATE $\mathcal{L}_{\text{SRL}}\gets -\mathcal{M}_{\text{RM}}(\hat{I}_{0}, I^s_{ref})$ // Calculate SRL loss with negative reward
%     \STATE $\mathcal{L}\gets \lambda\mathcal{L}_{\text{Pre}} + \mathcal{L}_{\text{SRL}}$
%     \STATE $\theta\gets\mathcal{L}$ // Update parameters with $\mathcal{L}$
% \ENDFOR
% \end{algorithmic}\label{algorithmic}
% \end{algorithm}

\begin{algorithm}[tb]
\caption{Style Reward Learning (SRL) with Flow Matching}
\begin{algorithmic}[1]
\REQUIRE Customization model $\texttt{net}$ with pretrained parameters $\theta$; pretrain loss $\mathcal{L}_{\text{Pre}}$; reward loss $\mathcal{L}_{\text{SRL}}$; reward model $\mathcal{M}_{\text{RM}}$; balancing coefficient $\lambda$; noise-schedule steps $T$; SRL fine-tuning interval $[t_s,t_e]$; dataset $\mathcal{D}=\{(y,I_0,I^c_{\text{ref}},I^s_{\text{ref}})\}$, $y$ is prompt, $I_0$ is target image and $I^c_{ref},I^s_{ref}$ are reference content and style images (\Cref{uno_dataset})

\FOR{$(y,I_0,I^c_{\text{ref}},I^s_{\text{ref}})\in\mathcal{D}$}
    \STATE $\mathcal{L}_{\text{Pre}}\gets \texttt{net}_{\theta}(y,I_0,I^c_{\text{ref}},I^s_{\text{ref}})$ // calculate pretrain loss with \Cref{eq5}
    \STATE $t\sim\mathcal{U}(t_s,t_e)$ // pick a random time step in $[t_s,t_e]$
    \STATE $x_T\sim\mathcal{N}(\mathbf{0},\mathbf{I})$
    \FOR{$\tau=T,\dots,t+1$}
        \STATE $\hat{v}_{\tau}\gets\text{no-grad}(\texttt{net}_{\theta}(y,x_{\tau},I^c_{\text{ref}},I^s_{\text{ref}}))$
        \STATE $x_{\tau-1}\gets x_{\tau}-\hat{v}_{\tau}\Delta t$ // reverse-step update
    \ENDFOR
    \STATE $\hat{v}_{t}\gets\texttt{net}_{\theta}(y,x_{t},I^c_{\text{ref}},I^s_{\text{ref}})$
    \STATE $\hat{I}_0\gets\operatorname{decode}(x_{t}-\hat{v}_t\Delta t)$ // predict original image
    \STATE $\mathcal{L}_{\text{SRL}}\gets -\mathcal{M}_{\text{RM}}(\hat{I}_0,I^s_{\text{ref}})$ // calculate SRL loss with negative reward with \Cref{eq6}
    \STATE $\mathcal{L}\gets\mathcal{L}_{\text{Pre}}+\lambda\mathcal{L}_{\text{SRL}}$
    \STATE $\theta\gets\theta-\eta\,\nabla_{\theta}\mathcal{L}$ // update model parameters via gradient descent ($\eta$ is learning rate)
\ENDFOR
\end{algorithmic}\label{alg:flow_srl}
\end{algorithm}

==> tables/teaser_table.tex <==
\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{0.9} % 调整行间距
     \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{lc}
        \toprule
        \textbf{Scenarios} & \textbf{Prompt} \\
        \midrule
        Subject/Identity Driven Generation & (1) "The girl is riding a bike in the street." \\
                & (2) "The man is driving a car in the street." \\
                & (3) "A sophisticated gentleman exuding confidence. He is dressed in a 1990s brown plaid jacket with a \\
                & high collar, paired with a dark grey turtleneck. His trousers are tailored and charcoal in color, \\
                & complemented by a sleek leather belt. The background showcases an elegant library with \\
                & bookshelves, a marble fireplace, and warm lighting, creating a refined and cozy atmosphere. \\
                & His relaxed posture and casual hand-in-pocket stance add to his composed and stylish demeanor" \\ 
                & (4) "The woman is reading a book in a cafe." \\
        \midrule
        Subject/Identity Driven Stylization & (1) "Sketch style, a bowl with a mountain in the background." \\
              & (2) "Illustration style, a dog on the beach." \\
              & (3) "Transform to Picasso's style of work, Cubism." \\
              & (4) "Ghibli style, The woman rides a deer in the forest." \\
        \midrule
        Style Driven Generation & (1)"A shark." \\
              & (2) "Small boat in the lake." \\    
              & (3) "A beautiful woman." \\    
              & (4) "The top chef is stir-frying in the kitchen." \\    
        \midrule
        Multi-style Driven Generation & (1) "A beautiful woman." \\
              & (2) "A duck, with words read "USO",  "inspires creativity"." \\    
              & (3) "A man." \\    
        \midrule
        Style-subject Driven Generation & (1) "" \\
           (Layout-preserved)   & (2) "" \\
           & (3) "" \\
        \midrule
        Style-subject Driven Generation & (1) "A toy in the jungle." \\
           (Layout-shifted)   & (2) "A cat on the beach." \\
           & (3) "The woman gave an impassioned speech on the podium." \\
        \bottomrule
    \end{tabular}
    }
    \caption{Text prompts used in \Cref{teaser}.}\label{tab:teaser}
\end{table*}  
